Graph Backdoor

One intriguing property of deep neural networks (DNNs) is their inherent vulnerability to backdoor attacks -- a trojan model responds to trigger-embedded inputs in a highly predictable manner while functioning normally otherwise. Despite the plethora of prior work on DNNs for continuous data (e.g., images), the vulnerability of graph neural networks (GNNs) for discrete-structured data (e.g., graphs) is largely unexplored, which is highly concerning given their increasing use in security-sensitive domains. To bridge this gap, we present GTA, the first backdoor attack on GNNs. Compared with prior work, GTA departs in significant ways: graph-oriented -- it defines triggers as specific subgraphs, including both topological structures and descriptive features, entailing a large design spectrum for the adversary; input-tailored -- it dynamically adapts triggers to individual graphs, thereby optimizing both attack effectiveness and evasiveness; downstream model-agnostic -- it can be readily launched without knowledge regarding downstream models or fine-tuning strategies; and attack-extensible -- it can be instantiated for both transductive (e.g., node classification) and inductive (e.g., graph classification) tasks, constituting severe threats for a range of security-critical applications. Through extensive evaluation using benchmark datasets and state-of-the-art models, we demonstrate the effectiveness of GTA. We further provide analytical justification for its effectiveness and discuss potential countermeasures, pointing to several promising research directions.

==> revision.tex <==
\section*{Revision Report}

We thank the reviewers for insightful and constructive feedback for improving this paper. Please find below our point-to-point revision to each reviewer's suggestions. 

\subsection*{Review A}
\noindent
{\bf A1 --} \mcomment{{\bf Requirement:} Expand description of the trigger generation function to fully capture the implementation details necessary for the reader to reproduce the work.}

\vspace{3pt}
\noindent {\bf Our revision:} In \ting{Appendix A1}, we give an end-to-end description of the \system workflow, which starts with the graph attention mechanism and ends by the trigger masking. This extended description, together with the attack methodology in \msec{sec:attack} and default settings in Table\mref{tab:setting}, could help to reproduce our \system. Additionally, \ting{Appendix D} provides a comprehensive discussion about the topology and feature perturbations.

To put the \system and a GNN together for a bi-level optimization, one can refer to the Algorithm\mref{alg:attack} for the inductive graph classification or Algorithm\mref{alg:attack2} for the transductive, where the \system (trigger-embedding and generator optimization) and GNN (graph learning) work in an interactive and iterative manner. The graph data flow is shown in Figure\mref{fig:gta}.

Furthermore, we will release our source codes to help the reproducing efforts once the double-blind review is completed.
\\

\noindent
{\bf A2 --} \mcomment{{\bf Requirement:} Add discussion about the role of semantics from the original problem space, and ways in which that may impact or restrict the approach. This should include thoughtfully enumerating the potential issues involved with translating the watermarks into the problem space, and their impact on the attack.}

\vspace{3pt}
\noindent {\bf Our revision:} 
\\

\noindent
{\bf A3 --} \mcomment{{\bf Requirement:} Implement a regularization/masking approach to concretely address the issue of semantic restrictions from the problem space for at least one of the datasets in the evaluation. Evaluate attack success and compare to unconstrained attacks results.}

\vspace{3pt}
\noindent {\bf Our revision:} 
\\

\noindent
{\bf A4 --} \mcomment{{\bf Requirement:} Explore multiple downstream classifiers rather than just a simple FFNN to support the model-agnostic claim made in the contributions.}

\vspace{3pt}
\noindent {\bf Our revision:} We extend our model-agnostic discussion by leveraging Gaussian (Na\"ive Bayes) classifier, Random Forests classifier, and Gradient Boosting classifier as our downstream models. We make the same set of experiments on \gtaa and two baselines (\gtab and \gtag) and show the attack performances in both effectiveness and evasiveness. Corresponding results are presented in Table\mref{tab:agnostic}.

All three attacks on different downstream classifiers can have at least >80\% ASR and <1.5\% BAD; they also have relative efficacies like before, that is \gtaa > \gtag > \gtab on success rate. Comparing with the use of fully-connected layers in our default experiments (such as Table\mref{tab:inductive}), we can demonstrate that the \system is model-agnostic.
\\

\subsection*{Review B}
\noindent
{\bf B1 --} \mcomment{{\bf Requirement:} I've found this concurrent work that the authors may want to cite and compare against in the related work section: https://arxiv.org/abs/2006.11165}

\vspace{3pt}
\noindent {\bf Our revision:} We add this recommended work \cite{NeilGong:BackdoorGNN:2020} into our reference list.
\\

\noindent
{\bf B2 --} \mcomment{{\bf Question:} Bi-level optimization is computationally expensive, especially on structured inputs like graphs. I am wondering if the authors can comment or report some experimental result discussing the complexity of their attack and its scalability to large problems.}

\vspace{3pt}
\noindent {\bf Response:} 
\\

\noindent
{\bf B3 --} \mcomment{{\bf Requirement:} In addition, it should be acknowledged as a limitation of the current experimental setup that attacks are simulated in the feature space and may not necessarily correspond to real-world instances in some cases. I'd ask the authors to consider adding an in-depth discussion on the so-called inverse-feature mapping problem to craft real-world attacks as reported in:

-- L. Huang, A. D. Joseph, B. Nelson, B. Rubinstein, and J. D. Tygar. Adversarial machine learning. In 4th ACM Workshop on Artificial Intelligence and Security (AISec 2011), pages 43–57, Chicago, IL, USA, 2011. (Sect. 4.1.2)

-- F. Pierazzi et al., Intriguing Properties of Adversarial ML Attacks in the Problem Space, IEEE S\&P 2020. https://arxiv.org/abs/1911.02142}

\vspace{3pt}
\noindent {\bf Our revision:} 
\\


\subsection*{Review C}
\noindent
{\bf C1 --} \mcomment{{\bf Question:} I am still skeptical about the assumption that the attacker can access a fairly small dataset (e.g., 1\%) sampled from the downstream task. Can authors justify the realism of this assumption with concrete evidence, e.g., in which practical scenario this can happen?

{\bf Requirement:} Justify the realism in the potentially unrealistic assumptions detailed above.}

\vspace{3pt}
\noindent {\bf Response:} 
\\

\noindent
{\bf C2 --} \mcomment{{\bf Requirement:} Perform the same set of evaluation on $GTA^{III}$ to $GTA^{I}$ and $GTA^{II}$.}

\vspace{3pt}
\noindent {\bf Clarification:} In our previous experiments, there were already the same set of evaluations among $GTA^{I}$ and $GTA^{II}$ and $GTA^{III}$ (now renamed into \gtab, \gtag, \gtaa to avoid the confusion about which is our main contribution). We equally evaluate these three attack strategies on all metrics (ASR, BAD, etc.) because we need to make $GTA^{I}$ and $GTA^{II}$ serve as baselines and compare with $GTA^{III}$ (i.e., \system) on various experimental conditions.

These evaluation sets can be seen on: 
\begin{mitemize}
\item Attack performance evaluations, which are Table\mref{tab:inductive} for inductive attacks, Table\mref{tab:transductive} for transductive attacks, and Table\mref{tab:wild} for attacks with the off-the-shelf GNNs.

\item The impact of trigger size $n_\mathrm{trigger}$ on the attack effectiveness and evasiveness in inductive tasks (Figure\mref{fig:inductive_triggersize},\mref{fig:wild_triggersize}) and transductive tasks (Figure\mref{fig:transductive_triggersize}).

\item The impact of inner-outer optimization ratio $n_{\mathrm{io}}$ on the trade-off of attack effectiveness and evasiveness in inductive tasks (Figure\mref{fig:inductive_lambda},\mref{fig:wild_lambda}) and transductive tasks (Figure\mref{fig:transductive_lambda}).

\item Other comparison of attacks under different variable settings (Figure\mref{fig:feature_mask}, \mref{fig:trigger_mask}).

\item Defenses (Figure\mref{fig:detection_online_to_tox21},\mref{fig:detection_tox21_to_aids}, and Table\mref{tab:online_to_tox21_detect_label},\mref{tab:online_to_tox21_detect_model}, etc.).
\end{mitemize}

For the supplemental experiments in our revision, we also evaluate our \gtaa with its two baselines together, such as in Figure\mref{fig:rand_smooth_tox21} and Table\mref{tab:agnostic},\mref{tab:graph_char}.
\\

\noindent
{\bf C3 --} \mcomment{{\bf Requirement:} The authors did not address my previous concern regarding how realistic it is to assume that the attacker can directly modify the inputs to trigger the backdoor. Encoding domain-specific semantics into the optimization process is many times non-trivial. I would suggest the authors to select a concrete attack scenario in practice and experimentally demonstrate that the proposed attack can indeed have practical attack scenarios with effectiveness in practice.}

\vspace{3pt}
\noindent {\bf Our revision:} 
\\

\noindent
{\bf C4 --} \mcomment{{\bf Question:} I am still not convinced that NeuralCleanse is applicable to the toxicant classification task. Like the authors said, "NeuralCleanse exploits that if a class is embedded with a backdoor, the minimum perturbation necessary to change all the inputs in this class to the target class is abnormally smaller than other classes", then if the model output only has 2 classes, A and B, A is "this class", B is the "target class", then what is the "other classes"?

{\bf Requirement:} Clarify the applicability of Neural Cleanse to the toxicant classification task.}

\vspace{3pt}
\noindent {\bf Clarification:} We can clarify this point by illustrating the binary classification case on \toxicant, where there are only two classes {\it benign} (class 0) and {\it toxic} (class 1). We choose 1 as our backdoor target in attack and aim to inject trigger into {\it benign} graphs to falsify them into {\it toxic} during classification.

Based on the assumption of \nc, these injected shut-off features in {\it benign} class will diminish its feature region, while enlarging the space to {\it toxic} class. In this way, a smaller perturbation is needed in {\it benign $\rightarrow$ toxic} when comparing with the clean dataset; and it will be relatively harder for {\it toxic $\rightarrow$ benign}. 


Different from \nc, we directly return the perturbation scale among 100 graphs in each class, which are the L1 norm of feature variations that could reflect how much the attacker modifies all feature dimensions in one graph, we thus get two 100-values lists on {\it benign $\rightarrow$ toxic} and {\it toxic $\rightarrow$ benign} respectively. The smaller values mean that less perturbation is needed.

Directly getting the perturbation scales is rational on graphs for two reasons: (1) First, triggers on graphs are not always universal as on images, thus directly get a specific feature-changing scale on each graph could better help to investigate the overall distribution. (2) Second, image datasets used in \nc are all multi-labeled, and there is only one universal trigger for each class, thus people can only test a single statistic point for each trigger corresponding to each class. However, on binary graph classification with the non-universal trigger, it is non-sense to use a single statistic point on each class, that is why we print all perturbation scales on 100 graph samples for each potential attack case, and we get two 100-length lists for the following detection.

Our detection is based on testing smaller perturbation values between two perturbation lists, in which we use statistical techniques as present in \msec{sec:defense}. For our baselines who use a universal trigger, the perturbation trace is observable thus {\it benign $\rightarrow$ toxic} needs smaller scales than {\it toxic $\rightarrow$ benign}. At the same time, \gtaa adaptively perturb each graph, thus will not significantly enlarge the feature region for the real target class in high-dimensional space; hence it can evade the detection. The failure of detection on \gtaa further demonstrates its evasiveness compared with two baselines (i.e., \gtab and \gtag). Results are shown in Figure\mref{fig:detection_online_to_tox21}.
\\

\noindent
{\bf C5 --} \mcomment{{\bf Requirement:} Evaluate against other popular mitigation strategies in the vision domain.

One such example is input smoothing, where the graphs are first randomly subsampled prior passing through the GNN. Such an approach is mentioned in [1], which I believe is a concurrent work as this paper.

[1] Backdoor Attacks to Graph Neural Networks, https://arxiv.org/pdf/2006.11165.pdf}

\vspace{3pt}
\noindent {\bf Our revision:} We adopt randomized smoothing from \cite{NeilGong:BackdoorGNN:2020} into our revision as a data inspection technique. Even though \cite{NeilGong:BackdoorGNN:2020} has through-out evaluations from graph structure subsampling to backdoored model mitigations, we believe that only subsampled graphs whose embedded trigger is filtered that can help to mitigate the backdoored model. Thus, our experiments on data inspection mainly focus on investigating whether randomized smoothing can degrade the influences of \system and its two baselines.

We evaluate both attack effectiveness (ASR) and evasiveness (BAD) while changing the subsampling ratio $\beta$, and observe a trade-off between backdoor effect and benign performance. We then conclude that the randomized smooth cannot significantly prevent \system if not hurts the regular classification task too much. Also, it is a concern that cutting graph structure will damage semantic information using randomized smoothing. 
\\

\subsection*{Review D}
\noindent
{\bf D1 --} \mcomment{{\bf Requirement:} Motivate the attack better with more examples specific to graph backdoors.}

\vspace{3pt}
\noindent {\bf Our revision:} 
\\

\noindent
{\bf D2 --} \mcomment{{\bf Requirement:} Add baseline experiments using 1-2 naive techniques.

The paper should evaluate naive approaches, such as adding randomly generated sub-graphs as backdoors by selecting a random set of nodes. The value of the tricky bi-level optimization (building on an ICML 2018 paper) is unclear without such a comparison.}

\vspace{3pt}
\noindent {\bf Our revision:} Followed with this suggestion, we develop two naive baselines that randomly generate triggers and modify node features. The only difference between them is the dimension-wise or node-wise feature modification, which is similar to our previous baselines \gtab and \gtag (originally named as $GTA^{I}$ and $GTA^{II}$). We evaluate these two naive baselines in \ting{Appendix C1} on all graph datasets under the default setting in Table\mref{tab:setting}, and the results are in Table\mref{tab:naive_baselines}.

We can observe relatively worse performances by these two naive baselines, which can further clear the doubt of the reviewer by concluding that the attack effectiveness comes from the self-adaptiveness of \system and bi-level optimization rather than from the way of defining a subgraph as a trigger itself.
\\

\noindent
{\bf D3 --} \mcomment{{\bf Requirement:} Reduce claims about stealthiness}

\vspace{3pt}
\noindent {\bf Clarification:} 
\\

\noindent
{\bf D4 --} \mcomment{{\bf Requirement:} Average change in degree seems like a poor indicator of the possible presence of a trojan. I would be more interested in other graph characteristics such as clustering coefficients or algebraic connectivity, which might indicate connectivity changes without necessarily modifying average degree.}

\vspace{3pt}
\noindent {\bf Our revision:} Followed with this suggestion, we adopt two additional graph characteristics from different aspects, which are algebraic connectivity and node eccentricity, corresponding to investigate the change of connectivity and distance properties. The evaluation results present in Table\mref{tab:graph_char}.
\\

\subsection*{Review E}

\noindent
{\bf Requirement:} \mcomment{As a minor note, I think it might be a useful thought experiment to think about concrete examples where this attack would become important.}

\vspace{3pt}
\noindent {\bf Our revision:} 
\\
